Best Privacy Practice Recommendations for Global Audio Streaming Platforms

Spoon Radio is a rapidly growing global audio streaming platform which currently operates in South Korea, the United States, Japan as well as the Middle East and North Africa. The platform believes that its commitment to user privacy is an important competitive factor. As such, it aims to not just comply with existing privacy regulations in regions where it operates today but to also ensure that it anticipates likely evolution to these regulations and of user expectations. In doing so, Spoon Radio wants to ensure it is well prepared to continue its expansion into new markets. As part of an effort to inform the evolution of its data practices, Spoon Radio reached out to the Privacy Engineering Program at CMU and sponsored a capstone project in which two master's students in the Program worked with Spoon Radio personnel over the course of the 2021 Fall Semester. The present report summarizes best practice recommendations that have emerged from this collaboration. These best practices are a combination of practices that are already implemented or in the process of being implemented by Spoon Radio today as well as more aspirational recommendations, which are expected to help inform Spoon Radio's practices in the future. In this report, best practice recommendations are organized around four stages of the data life cycle: data collection, data storage, data usage, and finally data destruction. A separate section is devoted to content moderation, an area where platforms such as Spoon Radio need to reconcile considerations such as promoting freedom of expression with the need to create a safe and respectful environment that complies with applicable laws and respects relevant cultural values.

==> guide.tex <==
\subsection{Figures and Tables}
\paragraph{Positioning Figures and Tables} Place figures and tables at the top and bottom of columns. Avoid placing them in the middle of columns. Large figures and tables may span across both columns. Figure captions should be  below the figures; table heads should appear above the tables. Insert figures and tables after they are cited in the text. Use the abbreviation ``Fig.~\ref{fig}'', even at the beginning of a sentence.

\begin{table}[htbp]
\caption{Table Type Styles}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Table}&\multicolumn{3}{|c|}{\textbf{Table Column Head}} \\
\cline{2-4} 
\textbf{Head} & \textbf{\textit{Table column subhead}}& \textbf{\textit{Subhead}}& \textbf{\textit{Subhead}} \\
\hline
copy& More table copy$^{\mathrm{a}}$& &  \\
\hline
\multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
\end{tabular}
\label{tab1}
\end{center}
\end{table}

==> sections/statement.tex <==
CMU is not a privacy authority per say
This report is merely the recommendation of best practice

==> tables/access_control.tex <==
\begin{table}[!ht] \setlength\tabcolsep{5pt} % you can change 0.1pt to maximum 9 pt, as you asked for IEEE
\caption{Example of Recommended RBAC table}
\begin{center}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|l|l|l|}
\hline
 &
  \begin{tabular}[c]{@{}l@{}}Register API\\ (Program)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}PayPal\\ (Third Party Services)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Moderator Team\\ (Employee)\end{tabular} \\ \hline
Identification Data & Read, Write, Use & Read & Read      \\ \hline
Financial Data      & Read, Write, Use & Read & -         \\ \hline
Audio Data          & -                & -    & Read, Use \\ \hline
\end{tabular}%
}
\end{center}
\end{table}

==> tables/archived_data.tex <==
\begin{table*}[!ht] \setlength\tabcolsep{5pt} % you can change 0.1pt to maximum 9 pt, as you asked for IEEE
\caption{Recommendation for Data Archiving}
\begin{center}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|}
\rowcolor{gray!50}
\hline
\textbf{Purpose of Archiving}      & \textbf{Required Methods} & \textbf{Related Personal Information Item}                                           \\ \hline
Complete Financial Transaction             & encryption              & Financial information, Purchase records            \\ \hline
Case for Moderation Training       & Anonymized                & Chats, audio data of LIVE; Comment, audio data in CAST; messages, audio data in TALK \\ \hline
Case of Customer Service                   & Anonymized              & Message and information in customer service ticket \\ \hline
Fulfill legal obligation                   & N/A                     & Depends on authorities request                     \\ \hline
Market analysis                            & Anonymized, aggregation & Purchase history, behavior data                    \\ \hline
Inputs for Machine Learning Model          & Anonymized, aggregation & Purchase history, behavior data                    \\ \hline
Logs for debug and system recovery & Anonymized                & Depends on the functionality. Delete after the function is repaired                  \\ \hline
Archived data for improving security issue & Anonymized              & Depends on the functionality                       \\ \hline
\end{tabular}%
}
\end{center}
\end{table*}

==> tables/personal_data_elements.tex <==
\begin{table}[htbp]
\caption{Personal Data Elements Collected by an Audio Social Network}
% \begin{center}
\begin{tabular}{|p{0.25\linewidth}|p{0.30\linewidth}|p{0.30\linewidth}|}
\hline
\multicolumn{3}{|c|}{\textbf{Personal Data Elements}} \\
% \cline{2-4}
\hline
Full Name, Nickname/ Username & Profile Photo/ Photos the user includes in communication on the platform & Contents of Communications with Spoon Radio (emails or calls to Customer Service)\\
\hline 
Password & Voice Introduction & Audio Recordings and Live Streams\\
\hline
Email Address & Topics of Interest & Content and metadata for comments\\
\hline
Date of Birth/ Birth Year & Identification for verifying identity (could be a driver’s licence, a passport, a school ID, etc.) & Content and metadata for private messages sent to other users\\
\hline
Phone Number & Metadata for purchases & IP Address\\
\hline
Gender & Financial Information & Device and Software Information (web browser, operating system, phone carrier) \\
\hline
Interaction Details (pages viewed, language selection, searches conducted, people followed, etc. & Cookies/pixel tags (or does the entry on the left cover it) & Demographic information received from third parties if a user logs in through a third party (e.g. Facebook, Gmail, etc.)\\
\hline
\end{tabular}
\label{dataelements}
% \end{center}
\end{table}

==> tables/retention_schedule.tex <==
\begin{table*}[!ht] \setlength\tabcolsep{5pt} % you can change 0.1pt to maximum 9 pt, as you asked for IEEE
\caption{example of possible retention period recommendation table}
\begin{center}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|}
\rowcolor{gray!50}
\hline
\textbf{Personal Information Item} &
\textbf{When to Delete} &
\textbf{Reason} &
\textbf{Note} \\ \hline
Email from third parties &
  N/A &
  Essential for Login &
   \\ \hline
Gender from third parties &
  User modified in their account setting &
  The right to sexuality &
  Should allow user to leave it open and self input \\ \hline
Date of Birth from third parties &
  User modified in their account setting &
   &
  Should allow user to make it public or not \\ \hline
Profile Information from third parties &
  After creating account &
  No specific purpose to hold it &
   \\ \hline
Device Information from third parties &
  After creating account &
  No specific purpose to hold it &
   \\ \hline
Other personal information imported from third parties &
  After creating account &
  No specific purpose to hold it &
   \\ \hline
Purchase Record collected by third parties &
  N/A &
  Essential for financial transaction &
  Spoon should able to delete it \\ \hline
Ephemeral content (audio, chat) in LIVE session &
  7 days &
  \begin{tabular}[c]{@{}l@{}}Reasonable period for moderating,\\ Only hold if there’s necessary for moderating\end{tabular} &
  Delete once the moderator processed \\ \hline
Persistent content (audio, comments) in CAST episode &
  User delete the episode or comments &
   &
   \\ \hline
Persistent content (audio, messages) in TALK session &
  \begin{tabular}[c]{@{}l@{}}User delete specific content manually,\\ User request\end{tabular} &
   &
  \begin{tabular}[c]{@{}l@{}}Allow user to delete specific content in a TALK session,\\ Allow user to delete all content of certain TALK session\end{tabular} \\ \hline
Device Information &
  Delete after logout &
  No specific purpose to hold it &
   \\ \hline
Customer Service information &
  1 Year &
  Reasonable period for customer service record lookups &
   \\ \hline
Customer Service information collected by Zendesk &
  1 Year, User request &
  Obligation to third parties &
   \\ \hline
Information leaved in promotion event s &
  Delete after the event &
  No specific purpose to hold it &
   \\ \hline
Advertising information collected by Braze &
  1 Year, User request &
  Obligation to third parties &
   \\ \hline
Other information collected by Third Parties &
  User request &
  Obligation to third parties &
   \\ \hline
\end{tabular}%
}
\end{center}
\end{table*}

==> tables/use_personal_info.tex <==
\begin{table*}[!ht] \setlength\tabcolsep{5pt} % you can change 0.1pt to maximum 9 pt, as you asked for IEEE
\caption{Example Personal Information Table}
\begin{center}
\begin{tabular}{|l|l|l|l|l|}
\hline
Personal Information  & Collect Method & Purpose of Collection & Retention & Who can Access                        \\ \hline
Real Name             & User Input     & Identification        & N/A       & Social Network, Customer Service Team \\ \hline
Click on certain Link & cookie\_xxx    & Advertising           & 7 days    & Advertising Team, Google Analytic     \\ \hline
\end{tabular}%
\end{center}
\end{table*}

==> tables/use_services.tex <==
\begin{table*}[!ht] \setlength\tabcolsep{5pt} % you can change 0.1pt to maximum 9 pt, as you asked for IEEE
\caption{Example Services Table}
\begin{center}
\begin{tabular}{|l|l|l|l|}
\hline
Vendor                   & subgroup        & Cookies       & Cookie Used \\ \hline
\multirow{2}{*}{Zendesk} & zendesk.com     & xxx, yyy, zzz & 3rd Party   \\ \cline{2-4} 
                         & www.zendesk.com & www, uuu      & 3rd Party   \\ \hline
Spoon                    & spoon.com       & aaa           & 1st Party   \\ \hline
\end{tabular}%
\end{center}
\end{table*}

==> tables/use_vendor.tex <==
\begin{table*}[!ht] \setlength\tabcolsep{5pt} % you can change 0.1pt to maximum 9 pt, as you asked for IEEE
\caption{Example Third Party Vendor Table}
\begin{center}
\begin{tabular}{|l|l|l|l|l|}
\hline
Name    & Description           & Related Services                                    & Accessibility to Personal Info & Official Website \\ \hline
PayPal  & Financial Transaction & Cookie\_xxx, payment interface                      & Credit card number, Address    & ...              \\ \hline
Zendesk & Customer Service      & Tracker\_xxx, cookie\_yyy, customer service request & Request issue, Email, post     & ...              \\ \hline
\end{tabular}%
\end{center}
\end{table*}
